Strategic Linear Contextual Bandits

Motivated by the phenomenon of strategic agents gaming a recommender system to maximize the number of times they are recommended to users, we study a strategic variant of the linear contextual bandit problem, where the arms can strategically misreport privately observed contexts to the learner. We treat the algorithm design problem as one of mechanism design under uncertainty and propose the Optimistic Grim Trigger Mechanism (OptGTM) that incentivizes the agents (i.e., arms) to report their contexts truthfully while simultaneously minimizing regret. We also show that failing to account for the strategic nature of the agents results in linear regret. However, a trade-off between mechanism design and regret minimization appears to be unavoidable. More broadly, this work aims to provide insight into the intersection of online learning and mechanism design.

==> figures/counterexample.tex <==



==> figures/regret_manipulation_util_figure.tex <==
\begin{figure}[t]
     \centering
    \begin{subfigure}[t]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/feature_plot.png}
        \caption{Total amount of context manipulation $\tilde C = \sum_{t,i} \lVert x_{t,i}^* - x_{t,i} \rVert_2$ as the arms adapt to the learning algorithms across 20 epochs.}
     \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/arm_util_joint.png}
        \caption{The utilities of the arms as they adapt to OptGTM and LinUCB, respectively. We do \emph{not} average but plot the utilities for each of the 10 runs.}
     \end{subfigure}
     \caption{$K=4$ strategic arms interact with OptGTM and LinUCB over the course of 20 epochs. Each epoch lasts $T = 10k$ time steps. In epoch 0, all arms report their contexts truthfully. At the end of every epoch, the arms greedily adapt their reporting strategies to the respective algorithm using gradient ascent. } 
     \label{fig:regret} 
\end{figure} 



==> figures/separate_util_figure.tex <==

\begin{figure}[t]
     \centering
    \begin{subfigure}[t]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/feature_plot.png}
        \caption{Total amount of context manipulation $\tilde C = \sum_{t,i} \lVert x_{t,i}^* - x_{t,i} \rVert_2$ as the arms adapt to the learning algorithms across 20 epochs.}
     \end{subfigure}
      \hfill
    \begin{subfigure}[t]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/arm_util_linucb.png} 
        \caption{The heavily unstable utilities of the arms as they adapt to LinUCB. We do \emph{not} average but plot the utilities for each of the 10 runs.} 
     \end{subfigure}
     \hfill
    \begin{subfigure}[t]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/arm_util_optgtm.png} 
        \caption{The utilities of the arms as they adapt to OptGTM. We do \emph{not} average but plot the utilities for each of the 10 runs.} 
     \end{subfigure}
     \caption{All arms begin by reporting their contexts truthfully in epoch 0. The arms then greedily adapt their reporting strategy to the algorithm using gradient ascent. The arms are optimal roughly the same number of times. } 
     \label{fig:metrics} 
\end{figure}


==> sections/figure.tex <==

\tikzset{node distance=0.3cm and 0.3cm, % Minimum distance between two nodes. Change if necessary.
}

\begin{figure}[t]
\centering 
\begin{tikzpicture}[>=stealth]
\node (x1) {$x_i$};
\node[above right=of x1] (x2) {$x_{i,1}$};
\node[below right=of x1] (x3) {$x_{i,2}$};
\node[below right=of x2] (x4) {$x_{i+1}$};

%empty nodes
\node[above left=of x1] (x5) {};
\node[below left=of x1] (x6) {};

\node[above right=of x4] (x7) {};
\node[below right=of x4] (x8) {};


\draw[-to] (x1) edge (x2);
\draw[-to] (x1) edge (x3);
\draw[-to] (x2) edge (x4);
\draw[-to] (x3) edge (x4);

\draw[-to] (x5) edge (x1);
\draw[-to] (x6) edge (x1);

\draw[-to] (x4) edge (x7);
\draw[-to] (x4) edge (x8);

\end{tikzpicture}
\caption{Figure Caption.}
\label{figure:figure1}
\end{figure}



==> sections/incentive_compatbility.tex <==


\section{The Necessity \emph{and} Impossibility of Incentive-Compatibility} \label{section:incentive_compatbility}
% \section{The Necessity of Aligning Incentives} 



Remarkably, we find that \emph{incentive-unaware} algorithms generally fail to be no-regret, while at the same time any precisely \emph{incentive-compatible} algorithm also suffers linear regret. 

  

We call a problem instance \emph{trivial} if the algorithm that selects an arm uniformly at random every round achieves sublinear regret. Conversely, we call a problem instance \emph{non-trivial} if the uniform selection strategy suffers linear expected regret. We show that being incentive-unaware generally leads to linear regret (even when the learner has prior knowledge of~$\theta^*$). 
\begin{prop}\label{lemma:incentive_unaware_greedy}
    On any non-trivial problem instance, the incentive-unaware greedy algorithm that in round $t$ plays $i_t = \argmax_{i \in [K]} \langle \theta^*, x_{t,i} \rangle$ (with ties broken uniformly) suffers linear regret $\Omega(T)$ when the arms act according to any Nash equilibrium under the incentive-unaware greedy algorithm.   

    Similarly, algorithms for stochastic linear contextual bandits (LinUCB \cite{chu2011contextual, abbasi2011improved}) and algorithms for linear contextual bandits with adversarial context corruption (RobustBandit \cite{ding2022robust}) suffer linear regret when the arms act according to any Nash equilibrium that the algorithms induce.  %\footnote{Unfortunately, existing work on adversarial linear contextual bandits \cite{neu2020efficient, liu2024bypassing, olkhovskaya2024first} cannot be mapped to our problem formulation, since they consider an adversarially chosen ``loss vector'' and assume correct contexts.} 
\end{prop}

\begin{proof}[Proof Sketch]
    Let $\tilde x := \argmax_{\lVert x \rVert_2 \leq 1} \langle \theta^*, x \rangle$. We show that the pure strategy profile, where every arm $i$ plays the strategy $x_{t, i} = \tilde x$ for all $t \in [T]$ is the unique Nash equilibrium under the incentive-unaware greedy algorithm. Under these arm strategies, actions in $\mathcal{X}_t$ become indistinguishable so that the greedy selection becomes uniform, thereby accumulating linear regret. %%%
    For the other algorithms, we also find that the only Nash equilibrium lies in strategies that myopically maximize the probability of being selected in every round. This once again leads to linear regret in all non-trivial problem instances given that ties are broken uniformly.   
    % In particular, any estimates of $\theta^*$ will be incorrect and the arms will be indistinguishable.  
    A complete proof is provided in Appendix~\ref{appendix:proof_incentive_unaware}.
\end{proof} 


We now show that it is \emph{impossible} to be incentive-compatible while minimizing regret. Here, an online learning algorithm is called \emph{incentive-compatible} if it is in each agent's best interest to be truthful, i.e., if reporting the true features every round is maximizing each arm's utility \citep{dekel2010incentive, mansour2015bayesian, freeman2020no}. Formally, $M$ is called incentive-compatible if there exists a Nash equilibrium $\bx \in \NE(M)$ such that $x_{t,i} = x_{t,i}^*$ for all $(t, i) \in [T] \times [K]$.  

\begin{prop}\label{lemma:incentive-compatible} 
    For any incentive-compatible algorithm there exists a problem instance such that the algorithm suffers linear regret for every Nash equilibrium of the arms. 
\end{prop}
% There exists no incentive-aware algorithm that achieves sublinear regret in every non-trivial problem instance. 
\begin{proof}[Proof Sketch.] 
    
    Suppose that there exists an incentive-compatible algorithm $\cA$ which achieves $o(T)$ regret under some Nash equilibrium of the arms. We will lead this to a contradiction by showing that either arms are not truthful or $\cA$ must select arms independently of the context of each round. Suppose that the algorithm's decision depends on the observed action set $X_T$ in round $T$. 
    If the selection is not uniform, then for each arm there is some action $x_{T,i}$ that maximizes its selection probability which is not equal to $x^*_{T,i}$ for some problem instance.\comment{[CD: I do not see why the previous sentence is true. Isn't it the premise that $x^*$ (and M) are in a NE, so deviating from it cannot be better?]} Since $\cA$ is incentive-compatible, it must therefore hold that $\cA$ selects an arm at round $T$ uniformly at random. Now, in round $T-1$, the same happens where the crucial observation is that misreporting features a single time is statistically undetectable for any algorithm. Hence, if an arm is untruthful only in round $T-1$ it can have no consequences for the selection in round $T$. As a result, $\cA$ must also make a decision independent of $X_{T-1}$ in round $T-1$, otherwise the dominant strategy for the arms would be to report $x_{T-1, i} \neq x_{T-1, i}^*$ such that their selection probability is maximized. Continuing the argument in this fashion, we see that in any NE some arm will misreport at least one time or $\cA$ will only make decisions independent of $X_1, \dots, X_T$. \textcolor{purple}{This proof is actually not that easy to do rigorously.} 
\end{proof} 

While Lemma~\ref{lemma:incentive_unaware_greedy} suggests that we must align the arms' incentives in order to achieve low regret, Lemma~\ref{lemma:incentive-compatible} on the other hand tells us that being incentive-compatible \emph{and} no-regret is impossible. 
This suggests that to achieve sublinear regret we must design \emph{approximately incentive-compatible} algorithms, for which the equilibrium arm strategies are asymptotically, approximately truthful, i.e., the total manipulation of the arms is bounded by some function decreasing in~$T$. If said difference is sufficiently small, we may achieve sublinear regret nonetheless.  


\begin{remark}
    Interestingly, we can design an incentive-compatible no-regret algorithm in the fully deterministic case, where $\theta^*$ is known a priori as well as the reward observations subject to \emph{no} noise (see Appendix~\ref{appendix:incentive_compatible}). This suggests that the trade-off between incentive-compatibility and regret minimization truly stems from the learner's uncertainty about both, the environment \emph{and} the arm strategies. 
\end{remark}


In a certain sense, the \emph{revelation principle} is violated in our setting. In fact, the revelation principle can be expected to fail under various kinds of uncertainty about environment and/or strategies besides the situation we study here.   
